Note about the complexity of the acyclic orientation with parity constraint problem

Let $G = (V, E)$ be a connected graph, and let $T$ in $V$ be a subset of vertices. An orientation of $G$ is called $T$-odd if any vertex $v \in V$ has odd in-degree if and only if it is in $T$. Finding a T -odd orientation of G can be solved in polynomial time as shown by Chevalier, Jaeger, Payan and Xuong (1983). Since then, $T$-odd orientations have continued to attract interest, particularly in the context of global constraints on the orientation. For instance, Frank and Kir\'aly (2002) investigated $k$-connected $T$-odd orientations and raised questions about acyclic $T$-odd orientations. This problem is now recognized as an Egres problem and is known as the "Acyclic orientation with parity constraints" problem. Szegedy ( 005) proposed a randomized polynomial algorithm to address this problem. An easy consequence of his work provides a polynomial time algorithm for planar graphs whenever $|T | = |V | - 1$. Nevertheless, it remains unknown whether it exists in general. In this paper we contribute to the understanding of the complexity of this problem by studying a more general one. We prove that finding a $T$-odd acyclic orientation on graphs having some directed edges is NP-complete.

==> preambule/bibliography.tex <==

% Toute la doc de biblatex est ici : 
% https://mirrors.ibiblio.org/CTAN/macros/latex/contrib/biblatex/doc/biblatex.pdf


%biber ./fileName.tex
%pdfLaTeX ./fileName.tex
%biber ./fileName.tex



% use for bibliography
\usepackage[
	backend=biber,        % compilateur par défaut pour biblatex
	backref=false,         % ajoute des liens dans les bibliographies
	sorting=none,          % trier par nom, année, titre
	citestyle= numeric,   % style de citation auteur-année
	bibstyle= numeric,    % style de bibliographie numérique
    doi=false,            % affiche les liens DOI
    isbn=false,           % affiche les numéros ISBN
    url=false,            % affiche les liens URLfirstinits=true, % affiche les initiales des prénoms    
    giveninits=true,      % affiche les initiales des prénoms
    eprint=false,         % affiche les liens arXiv
    hyperref=true,        % ajoute des liens hypertexte
    alldates=year,        % affiche seulement l'année
    datezeros=true,       % affiche les zéros dans les dates
    natbib=true,          % permet d'utiliser natbib
]{biblatex}


\renewbibmacro*{issue+date}{%
	\iffieldundef{year}
	{} % Ne rien afficher
	{\printtext[parens]{\printfield{year}}} % Sinon, afficher year entre parenthèses
}

\AtEveryBibitem{\clearfield{pagetotal}}
\AtEveryBibitem{\clearfield{visited}}
\renewbibmacro{in:}{%
    \ifentrytype{article}
    {}
    {\bibstring{in}%
        \printunit{\intitlepunct}}}


\DeclareCiteCommand{\cite} % cite author + (date) + [index]
    {\boolfalse{citetracker}%
	\boolfalse{pagetracker}%
	\usebibmacro{prenote}}
    {\ifciteindex
        {\indexnames{labelname}} 								% si index a des paramètres/labels on les index
        {}														% sinon rien
	\printnames{labelname}										% on affiche le nom de l'auteur
	\iffieldundef{year}											% si le champ "year" du label n'est pas défini
		{}														% on ne fait rien
		{\setunit{\printdelim{nonameyeardelim}} 				% sinon on ajoute un espace
		\printfield[parens]{year}}								% et on affiche l'année entre parenthèses
	\setunit{\printdelim{nonameyeardelim}}
	\printtext[bibhyperref]{									% on affiche le texte en hyperlien vers la biblio
		\printtext[brackets]{\printfield{labelnumber}}}}		% on affiche le numéro de la citation entre crochets
	{\multicitedelim}
	{\usebibmacro{postnote}}


\DeclareCiteCommand{\citenum} % [index]
    {\boolfalse{citetracker}%
	\boolfalse{pagetracker}%
	}
	{\printtext[bibhyperref]{
		\printtext[brackets]{\printfield{labelnumber}}}}  % Affiche le numéro de citation entre crochets
    {\multicitedelim}  % Séparateur pour les citations multiples
    {}

% Chatgpt option (other example)
\DeclareCiteCommand{\citeold} % cite author + [index]
	{\usebibmacro{prenote}} % Avant la citation
	{\printnames{author}% Imprime les noms des auteurs
	 \addspace% Espace après l'auteur
	 \printdate% Imprime l'année entre parenthèses
	 \addspace% Espace après l'année
	 \printtext[bibhyperref]{
		\printtext[brackets]{\printfield{labelnumber}}}} % Numéro de la référence entre crochets
	{\multicitedelim} % Délimiteur si plusieurs citations
	{\usebibmacro{postnote}} % Après la citation

\DeclareCiteCommand{\citetitle}
	{\boolfalse{citetracker}%
	\boolfalse{pagetracker}%
	\usebibmacro{prenote}}
	{\ifciteindex
		{\indexfield{indextitle}}
		{}%
		\printtext[bibhyperref]{\printfield[citetitle]{labeltitle}}}
	{\multicitedelim}
	{\usebibmacro{postnote}}

\DeclareCiteCommand{\citeauthor}
	{\boolfalse{citetracker}%
	\boolfalse{pagetracker}%
	\usebibmacro{prenote}}
	{\ifciteindex
		{\indexnames{labelname}}
		{}%
		\printtext[bibhyperref]{\printnames{labelname}}}
	{\multicitedelim}
	{\usebibmacro{postnote}}


\DeclareFieldFormat{backrefparens}{#1.}


% Bibliographie filtrée pour les sciences de l'éducation
\defbibfilter{education}{
  	keyword={education}
}

\defbibfilter{graph}{
  	keyword={graph}
}

\defbibfilter{no_educ}{
  	not keyword={education}
}


%\addbibresource{/home/petiteam/Documents/These/Papers/Paper In progress/CSI-2A/CSI-2A.bib} %PC IF
\addbibresource{biblio.bib}
